SCOI: Syntax-augmented Coverage-based In-context Example Selection for Machine Translation

In-context learning (ICL) greatly improves the performance of large language models (LLMs) on various down-stream tasks, where the improvement highly depends on the quality of demonstrations. In this work, we introduce syntactic knowledge to select better in-context examples for machine translation (MT). We propose a new strategy, namely Syntax-augmented COverage-based In-context example selection (SCOI), leveraging the deep syntactic structure beyond conventional word matching. Specifically, we measure the set-level syntactic coverage by computing the coverage of polynomial terms with the help of a simplified tree-to-polynomial algorithm, and lexical coverage using word overlap. Furthermore, we devise an alternate selection approach to combine both coverage measures, taking advantage of syntactic and lexical information. We conduct experiments with two multi-lingual LLMs on six translation directions. Empirical results show that our proposed SCOI obtains the highest average COMET score among all learning-free methods, indicating that combining syntactic and lexical coverage successfully helps to select better in-context examples for MT. Our code is available at https://github.com/JamyDon/SCOI.

==> table/OrderSim-dep.tex <==
\begin{table*}[htbp]
\small
  \centering
    \begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}[4]{*}{\textbf{Order}} & \multirow{2}[4]{*}{\textbf{Measure}} & \multicolumn{3}{c}{\textbf{Into EN}} & \multicolumn{3}{c}{\textbf{Out of EN}} & \multirow{2}[4]{*}{\textbf{Avg.}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}          &       & \textbf{DE} & \textbf{FR} & \textbf{RU} & \textbf{DE} & \textbf{FR} & \textbf{RU} &  \\
    \midrule
    \multirow{2}[2]{*}{Word First} & Cosine Similarity & 63.96 & 70.86 & 53.84 & 44.14 & 55.16 & 45.49 & 55.58 \\
          & Normalized Distance & 64.45 & 70.64 & 53.76 & 45.39 & \textbf{55.91} & 45.63 & 55.96 \\
    \midrule
    \multirow{2}[2]{*}{Syntax First} & Cosine Similarity & 64.35 & \textbf{71.54} & 53.89 & \textbf{45.41} & 55.36 & 46.06 & 56.10 \\
          & Normalized Distance & \textbf{64.67} & 71.26 & \textbf{54.08} & 44.87 & 55.31 & \textbf{46.47} & \textbf{56.11} \\
    \bottomrule
    \end{tabular}
  \caption{COMET scores of 4-shot ICL performance of different orders of alternating and measures of coverage. The highest scores are in \textbf{bold} text.}
  \label{tab:ordersim}
\end{table*}

==> table/case-simp.tex <==
\begin{table}[htbp]
  \centering
  \scalebox{0.8}{
    \begin{tabular}{c|l}
    \hline
    \textbf{Input (DE)} & \makecell[l]{Nach einer Woche voller Verluste in der\\ Zwischenwahl erzählte Bush dem Publikum\\ von \textbf{der Ausweitung des Handels in Asien}.} \\
    \hline
    \textbf{Gold (EN)} & \makecell[l]{After a week of losses in the midterm\\ election, Bush told an audience about \textbf{the}\\ \textbf{expansion of trade in Asia}.} \\
    \hline
    \textbf{BM25} & \makecell[l]{After a week of losses in the mid-election\\ campaign, President Bush told his audience\\ \textbf{that trade in Asia had been expanded}.} \\
    \hline
    \textbf{Ours} & \makecell[l]{After a week of losses in the mid-term\\ election, Bush told the audience about \textbf{the}\\ \textbf{expansion of trade in Asia}.} \\
    \hline
    \end{tabular}}
  \caption{A "DE-EN" translation example comparing the system outputs of BM25 and our method.}
  \label{tab:casesimp}
\end{table}


==> table/mode-comet.tex <==
\begin{table*}[htbp]
\small
  \centering
    \begin{tabular}{ccccccccc}
    \toprule
    \multirow{2}[4]{*}{\textbf{Mode}} & \multirow{2}[4]{*}{\textbf{Feature}} & \multicolumn{3}{c}{\textbf{Into EN}} & \multicolumn{3}{c}{\textbf{Out of EN}} & \multirow{2}[4]{*}{\textbf{Avg.}} \\
\cmidrule(lr){3-5}\cmidrule(lr){6-8}          &       & \textbf{DE} & \textbf{FR} & \textbf{RU} & \textbf{DE} & \textbf{FR} & \textbf{RU} &  \\
    \midrule
    Top-$k$ (BM25) & Word & 63.21 & 71.36 & 52.48 & 44.13 & 55.54 & 44.58 & 55.22 \\
    \midrule
    Top-$k$ (Syntax) & Syntax & 64.15 & 70.79 & 53.71 & 43.22 & 54.75 & 46.49 & 55.52 \\
    \midrule
    \multirow{3}[2]{*}{DPP} & Word-D  & 63.99 & 71.44 & 52.87 & 41.99 & 54.18 & 44.55 & 54.84 \\
          & Word-D + Word-R & 63.88 & 71.31 & 53.21 & 43.95 & 55.59 & 45.36 & 55.55 \\
          & Word-D + Syntax-R & 63.64 & 70.71 & 53.65 & 43.61 & 55.55 & 45.48 & 55.44 \\
    \midrule
    \multirow{2}[2]{*}{Coverage} & Word  & 64.44 & \textbf{71.52} & 53.33 & 43.99 & 55.52 & 46.22 & 55.84 \\
          & Syntax & 63.84 & 70.95 & 53.30 & 42.55 & \textbf{56.25} & \textbf{46.82} & 55.62 \\
    \midrule
    Combined Coverage (\textit{proposed}) & Word + Syntax & \textbf{64.67} & 71.26 & \textbf{54.08} & \textbf{44.87} & 55.31 & 46.47 & \textbf{56.11} \\
    \bottomrule
    \end{tabular}
  \caption{COMET scores of 4-shot ICL performance of different selection modes. "\textbf{Feature}" refers to the aspect(s) of features used during selection ("D" and "R" in the "DPP" mode refers to "diversity" and "relevance" respectively). \textbf{"Avg.}" refers to the average score across all 6 directions. The highest scores are in \textbf{bold} text.}
  \label{tab:mode-comet}
\end{table*}
